Persistent Memory I/O Primitives

I/O latency and throughput is one of the major performance bottlenecks for disk-based database systems. Upcoming persistent memory (PMem) technologies, like Intel's Optane DC Persistent Memory Modules, promise to bridge the gap between NAND-based flash (SSD) and DRAM, and thus eliminate the I/O bottleneck. In this paper, we provide one of the first performance evaluations of PMem in terms of bandwidth and latency. Based on the results, we develop guidelines for efficient PMem usage and two essential I/O primitives tuned for PMem: log writing and block flushing.

==> figures/page_flush/mt_scale_cl/scalar.tex <==

\begin{tikzpicture}
   \begin{axis}[
      width=\textwidth/\flushPageChartScale,
      height=4cm,
      xlabel={Dirty cache line count \vphantom{[]}},
      axis lines=left,
      ymin=0, ymax=3.4,
      legend columns=3,
      mark repeat = 4,
      mark phase = 1,
      xtick={16,48,128,256},
      yticklabel={%
      	\ifthenelse{\equal{\tick}{0.0}}
      	{0}
      	{\SI[round-mode=places, round-precision=0]{\tick}{K}}
      },
      ]

      \addplot[samples=1, domain=0:6, gray, name path=three, forget plot] coordinates {(48,0)(48,0.6)};

      % Micro log
      \addplot[thick,color=color1,mark=triangle] file {figures/page_flush/mt_scale_cl/data/scalar_micro.data};

      % Shadow (only dirty resident)
      \addplot[thick,color=color4,mark=x] file {figures/page_flush/mt_scale_cl/data/scalar_shadow.data};

      % Shadow (all resident)
      \addplot[thick,color=color2,mark=o] file {figures/page_flush/mt_scale_cl/data/scalar_shadow_resident.data};

   \end{axis}
\end{tikzpicture}


==> figures/page_flush/scale_threads/scalar.tex <==

\begin{tikzpicture}
   \begin{axis}[
      width=\textwidth/\flushPageChartScale,
      height=4cm,
      xlabel={Thread count \vphantom{[]}},
      axis lines=left,
      ymin=0, ymax=2.2,
      xmin=1, xmax=25,
      legend columns=3,
      xtick={1,5,10,15,20,24},
      yticklabel={%
      	\ifthenelse{\equal{\tick}{0.0}}
      	{0}
      	{\SI[round-mode=places, round-precision=0]{\tick}{K}}
      },
      ytick={0,1,2},
      ]

      % Micro log
      \addplot[thick,color=color1,mark=triangle] file {figures/page_flush/scale_threads/data/scalar_micro.data};

      % Shadow (only dirty resident)
      \addplot[thick,color=color4,mark=x] file {figures/page_flush/scale_threads/data/scalar_shadow.data};

      % Shadow (all resident)
      \addplot[thick,color=color2,mark=o] file {figures/page_flush/scale_threads/data/scalar_shadow_resident.data};

      \node[right, color1] at (10.0,1.55) {\small 11};
      \node[right, color4] at (9.0,0.25) {\small 10};
      \node[right, color2] at (10.0,0.70) {\small 11};

   \end{axis}
\end{tikzpicture}


==> figures/page_flush/st_scale_cl/scalar.tex <==

\begin{tikzpicture}
   \begin{axis}[
      width=\textwidth/\flushPageChartScale,
      height=4cm,
      xlabel={Dirty cache line count \vphantom{[]}},
      ylabel={\si{Pages\per\second} \vspace{1mm}},
      axis lines=left,
      ymin=0, ymax=500,
      legend columns=3,
      mark repeat = 4,
      mark phase = 1,
      xtick={16,48,128,256},
      legend cell align={left},
      legend to name={page_flush_ledgend},
      legend style={at={(0.5,0.8)},anchor=west},
      yticklabel={%
      	\ifthenelse{\equal{\tick}{0.0}}
      	{0}
      	{\SI[round-mode=places, round-precision=0]{\tick}{K}}
      },
      ]
      \legend{\textmu{}Log, CoW, CoW (all resident)}

      \addplot[samples=1, domain=0:6, gray, name path=three, forget plot] coordinates {(48,0)(48,180)};

      % Micro log
      \addplot[thick,color=color1,mark=triangle] file {figures/page_flush/st_scale_cl/data/scalar_micro.data};

      % Shadow (only dirty resident)
      \addplot[thick,color=color4,mark=x] file {figures/page_flush/st_scale_cl/data/scalar_shadow.data};

      % Shadow (all resident)
      \addplot[thick,color=color2,mark=o] file {figures/page_flush/st_scale_cl/data/scalar_shadow_resident.data};

   \end{axis}
\end{tikzpicture}

